Pretraining Text Encoders with Adversarial Mixture of Training Signal Generators

We present a new framework AMOS that pretrains text encoders with an Adversarial learning curriculum via a Mixture Of Signals from multiple auxiliary generators. Following ELECTRA-style pretraining, the main encoder is trained as a discriminator to detect replaced tokens generated by auxiliary masked language models (MLMs). Different from ELECTRA which trains one MLM as the generator, we jointly train multiple MLMs of different sizes to provide training signals at various levels of difficulty. To push the discriminator to learn better with challenging replaced tokens, we learn mixture weights over the auxiliary MLMs' outputs to maximize the discriminator loss by backpropagating the gradient from the discriminator via Gumbel-Softmax. For better pretraining efficiency, we propose a way to assemble multiple MLMs into one unified auxiliary model. AMOS outperforms ELECTRA and recent state-of-the-art pretrained models by about 1 point on the GLUE benchmark for BERT base-sized models.

==> Tables/ablation.tex <==

% \begin{table*}[t]
% \centering
% \small
\begin{wraptable}{r}{0.6\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llll}
\hline
\multirow{2}{*}{\textbf{Group}} & \multirow{2}{*}{\textbf{Method}} & \textbf{MNLI-(m/mm)} & \textbf{SQuAD 2.0 EM/F1} \\
\hline
& \model{}$_\text{Base}$ & 88.9/88.7 & 84.2/87.2  \\ 
\hline
\textbf{Curriculum} & w. random layer & 88.6/88.3 & 83.6/86.6 \\
\textbf{Setup} & w. layer switch & 88.6/88.4 & 83.3/86.2 \\
\hline
\textbf{Adversarial} & - adv. train & 88.7/88.5 & 83.9/86.8 \\
\textbf{Setup} & + adv. MLM & 88.6/88.7 & 84.2/87.2 \\
\hline
\textbf{Multi-MLM} & - stop grad. & 88.5/88.6 & 83.6/86.6 \\
\textbf{Setup} & w. separate MLM gen. & 88.8/88.7 & 83.4/86.5 \\
\hline
\textbf{Backbone} & - multi-MLM - adv. train & 88.5/88.2 & 83.1/86.0 \\
\hline
\end{tabular}
}
\caption{
Ablations on MNLI and SQuAD 2.0 development set that eliminate (-), add (+) or switch (w.) one component.
}
\label{tab:ablation} 
% \end{table*}
\end{wraptable}


==> Tables/gen_layer_mnli.tex <==
\setlength{\tabcolsep}{4pt}
\begin{wraptable}{r}{0.3\textwidth}
    \centering
    % \vspace{-0.3cm}
%  \input{Tables/clm_sim_squad}
 \resizebox{\textwidth}{!}{
 \begin{tabular}{c|cc}
\toprule 
\textbf{Gen. Layers} & \textbf{MNLI-m} & \textbf{GLUE Avg.}
\\ 
\midrule
2 & 87.9 &  \\
4 & 88.5 &  \\
8 & 88.2 & \\
\midrule
ELECTRA & 86.9 & 85.5 \\
\bottomrule
\end{tabular}
}
\caption{Downstream task fine-tuning scores on MNLI (matched) and GLUE average of the discriminator when pretrained with generators of different sizes.
} 
\label{tab:gen_layer_mnli}
\end{wraptable}
\setlength{\tabcolsep}{6pt}

==> Tables/probing.tex <==

% \begin{table}[t]
% \centering
% \begin{tabular}{lllllllll}
% \toprule
%         & pos  & nonterminal & dep  & ner  & srl  & coref & spr2 & semeval \\
% \midrule
% 4 layer & 93.7 & 75.0        & 88.8 & 93.6 & 80.9 & 80.0  & 79.8 & 74.5    \\
% 6 layer & 94.7 & 76.2        & 89.4 & 94.8 & 81.6 & 81.7  & 81.3 & 75.8    \\
% 8 layer & 94.3 & 76.3        & 89.5 & 94.9 & 82.3 & 81.7  & 80.2 & 75.0    \\
% \bottomrule
% \end{tabular}
% \end{table}
\begin{wraptable}{r}{0.4\textwidth}
\centering
\resizebox{\textwidth}{!}{
% \begin{table}[t]
\begin{tabular}{llll}
\toprule
Tasks           & 4 layer & 6 layer & 8 layer \\
\midrule
POS         & 93.7    & \textbf{94.7}    & 94.3    \\
Consts. & 75.0    & 76.2    & \textbf{76.3}    \\
Deps.         & 88.8    & 89.4    & \textbf{89.5}    \\
Entities         & 93.6    & 94.8    & \textbf{94.9}    \\
SRL         & 80.9    & 81.6    & \textbf{82.3}    \\
Coref.       & 80.0    & \textbf{81.7}    & \textbf{81.7}    \\
SPR2        & 79.8    & \textbf{81.3}    & 80.2    \\
Relations     & 74.5    & \textbf{75.8}    & 75.0   \\
\bottomrule
\end{tabular}
}
% \end{table}
\caption{Experiment results of $4$/$6$/$8$-layer MLM generator on eight probing tasks. Generators of different sizes are good at different tasks.}
\label{tab:probe}
\end{wraptable}

